LLaMAX: Scaling Linguistic Horizons of LLM by Enhancing Translation Capabilities Beyond 100 Languages

Large Language Models (LLMs) demonstrate remarkable translation capabilities in high-resource language tasks, yet their performance in low-resource languages is hindered by insufficient multilingual data during pre-training. To address this, we conduct extensive multilingual continual pre-training on the LLaMA series models, enabling translation support across more than 100 languages. Through a comprehensive analysis of training strategies, such as vocabulary expansion and data augmentation, we develop LLaMAX. Remarkably, without sacrificing its generalization ability, LLaMAX achieves significantly higher translation performance compared to existing open-source LLMs (by more than 10 spBLEU points) and performs on-par with specialized translation model (M2M-100-12B) on the Flores-101 benchmark. Extensive experiments indicate that LLaMAX can serve as a robust multilingual foundation model. The code \footnote{\url{https://github.com/CONE-MT/LLaMAX/.}} and the models \footnote{\url{https://huggingface.co/LLaMAX/.}} are publicly available.

==> EMNLP-2024/sections/4.approach_backup.tex <==
\section{Approach}
\subsection{Lexicons Augmentation}
\subsubsection{Build Multilingual lexicons}
After collecting the bilingual lexicons from MUSE and PanLex, we considered integrating them into a multilingual lexicon. We loop through each bilingual lexicon, recording synonyms for each entry in the target language, aggregating synonyms from different languages together. In addition, we filter all punctuation in lexicons. We then construct a new multilingual lexicon in the following format for each entry:
\texttt{\{word\}\_\{lang\}}

\subsubsection{Synonyms Random Alignment}
Firstly, we convert the source sentence text to a list of words. For most languages, we split the source sentence with white space to a list of words. Especially for Chinese, we use Jieba to complete such operation. And then, for each pair of parallel data, we will randomly select a language from those supported by the lexicon and use a word-to-word translation method to translate original source sentence into the chosen language. 
If no synonym can be found in the selected language, we will retain the original word. Additionally, for words that have synonyms available, we will set a 90\% probability of replacement with the identified synonym. If multiple synonyms are found, one will be randomly chosen. Finally, this new translation will form new pseudo-parallel data with the original target language sentence.

\subsection{Pretraining Data}
Our data consists of two parts: parallel corpora and monolingual corpora, both sourced from public datasets. The parallel corpora are from FedMT dataset (organized from publicly available datasets on OPUS), and the monolingual corpora are from mc4. Both the parallel and monolingual corpora cover 102 languages, consistent with the languages supported by flores101. Additionally, to address the lack of parallel data for low-resource languages, we have expanded our dataset with a batch of pseudo-parallel data using a dictionary-enhanced method.

\subsubsection{Parallel Data}
Our parallel corpus involves 102 languages and 4200 language pairs, totaling 80G of data. For each language pair, Language A and Language B, each translation set is concatenated together with a space separating them as a single training data entry. Each direction, A->B and B->A, has a 50\% probability of occurrence. During training, the gradient of the entire data entry is calculated, not just the target sentence. For language pairs with fewer than 25,000 parallel corpus entries, we copy the original data three times to ensure that low-resource language pairs still have sufficient training data volume.

\subsubsection{Monolingual Data}
Our monolingual data includes the same 102 languages from mC4 and MADLAD, totaling 40,000,000 entries and 60G in size. For each piece of monolingual data, we set a block size of 512 to split it into multiple entries.

\subsubsection{Synthetic Data}
For low-resource languages with limited data, in addition to simply copying the original data multiple times, we also use dictionary-enhanced methods to construct pseudo-parallel corpora. Here, we utilize the Panlex and Muse dictionaries. We first translate 2 million sentences of monolingual English data from the Europarl corpus into 101 languages using the FedMT model. Then, for the low-resource language pairs that require enhancement, we use the translated corpora to construct pseudo-parallel corpora. To project low-resource languages into the same vector space as high-resource languages, 90\% of the words in the source sentence of each pseudo-parallel corpus entry are replaced with semantically equivalent words in a specified language (randomly chosen from one of the 101 languages other than the source language). If no translation is available for a word, the word from the original language is retained.

\subsection{Supervised Fine-Tuning (SFT) Data}
We construct our instruction data using publicly available data from the internet, primarily sourced from the following three origins: alpaca, aya-dataset, and FedMT.

\begin{description}
    \item[Alpaca] consists of 52k English instruction-following data, generated using OpenAI's text-davinci-003 model.
    \item[Aya-dataset] is a human-annotated multilingual instruction-following dataset. The dataset contains 204,000 entries and spans 65 languages, comprising 22 high-resource, 12 mid-resource, and 31 low-resource languages. It covers a range of tasks such as question answering, paraphrasing, and translation.
    \item[FedMT] is a multilingual translation dataset that covers 435 languages and 22,613 language pairs. We have sampled 1,000 data points from each of the 102 languages supported by flores101 and converted them into instruction data for translation tasks. The translation prompts are shown in Table~\ref{tab:translation_prompts}.
\end{description}
All instruction-following data use prompts recommended by alpaca as illustrated in Table~\ref{tab:non-empty_input} and Table~\ref{tab:empty_input}.


\begin{table*}[ht]  % [ht] 代表 "here", 尽量在当前位置显示表格
\centering
\begin{tabular}{|p{\textwidth}|}
\hline
Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \\
\hline
\textbf{Instruction:} \\
{instruction} \\
\hline
\textbf{Input:} \\
{input} \\
\hline
\textbf{Response:} \\
% Here response will be added. Make sure to add \\ at the end when adding the actual content.
\hline
\end{tabular}
\caption{examples with a non-empty input field}  % 添加表格标题
\label{tab:non-empty_input}
\end{table*}

\begin{table*}[ht]  % [ht] 代表 "here", 尽量在当前位置显示表格
\centering
\begin{tabular}{|p{\textwidth}|}
\hline
Below is an instruction that describes a task, paired with an input that provides further context. Write a response that appropriately completes the request. \\
\hline
\textbf{Instruction:} \\
{instruction} \\
\hline
\textbf{Response:} \\
% Here response will be added. Make sure to add \\ at the end when adding the actual content.
\hline
\end{tabular}
\caption{examples with a empty input field}  % 添加表格标题
\label{tab:empty_input}
\end{table*}



\begin{table*}[h]  % [ht] 代表 "here", 尽量在当前位置显示表格
\centering
\begin{tabular}{|p{\textwidth}|}
\hline
\textbf{Translation Prompts} \\
\hline
Translate the following sentences from [SRC] to [TGT]. \\
What do the following sentences mean in [TGT]? \\
Please provide the [TGT] translation for the following sentences. \\
Convert the subsequent sentences from [SRC] into [TGT]. \\
Render the listed sentences in [TGT] from their original [SRC] form. \\
Transform the upcoming sentences from [SRC] language to [TGT] language. \\
Change the given sentences from [SRC] to [TGT] format. \\
Turn the following sentences from their [SRC] version to the [TGT] version. \\
Adapt the mentioned sentences from [SRC] to the [TGT] language. \\
Transpose the next sentences from the [SRC] format to the [TGT] format. \\
Switch the specified sentences from their [SRC] form to [TGT] form. \\
Reinterpret the ensuing sentences from [SRC] to [TGT] language. \\
Modify the forthcoming sentences, converting them from [SRC] to [TGT]. \\
How can the subsequent sentences be interpreted in [TGT]? \\
What is the meaning of these sentences when translated to [TGT]? \\
In the context of [TGT], what do the upcoming sentences signify? \\
How would you express the meaning of the following sentences in [TGT]? \\
What is the significance of the mentioned sentences in [TGT]? \\
In [TGT], what do the given sentences convey? \\
When translated to [TGT], what message do these sentences carry? \\
What is the intended meaning of the ensuing sentences in [TGT]? \\
How should the following sentences be comprehended in [TGT]? \\
In terms of [TGT], what do the next sentences imply? \\
Kindly furnish the [TGT] translation of the subsequent sentences. \\
Could you supply the [TGT] translation for the upcoming sentences? \\
Please offer the [TGT] rendition for the following statements. \\
I'd appreciate it if you could present the [TGT] translation for these sentences. \\
Can you deliver the [TGT] translation for the mentioned sentences? \\
Please share the [TGT] version of the given sentences. \\
It would be helpful if you could provide the [TGT] translation of the ensuing sentences. \\
Kindly submit the [TGT] interpretation for the next sentences. \\
Please make available the [TGT] translation for the listed sentences. \\
Can you reveal the [TGT] translation of the forthcoming sentences? \\
\hline
\end{tabular}
\caption{List of Translation Prompts}  % 添加表格标题
\label{tab:translation_prompts}
\end{table*}

\section{Training}
Our pre-training is mainly divided into the following three stages.
\subsection{Pretrain}
\subsubsection{Stage1}
For parallel data, we sample 50,000 entries per language pair from FedMT. If a language pair has fewer than 50,000 entries, we make three copies of the original data. For monolingual data, we used sources from mC4 and MADLAD, sampling 400,000 sentences from each language, splitting the data into blocks with a block size of 512. After shuffling all the data, we train using Hugging Face Transformers on the DeepSpeed parallel architecture.
\subsubsection{Stage2}
For parallel data, we still sampled 50,000 entries for each language pair in FedMT. For pairs with fewer than 50,000 samples, we duplicated the original data and sampled from the corresponding synthetic data at a 1:1 ratio. For monolingual data, we continued sampling from mC4 and MADLAD but at a lower sampling rate compared to the parallel data. We reduced the count per language from 400,000 in the first round to 200,000.
\subsubsection{Stage3}
For some underperforming language pairs (sacrebleu < 20), we sampled parallel corpora from FedMT at a 2:1 ratio compared to better-performing pairs (700,000 for underperforming pairs and 350,000 for better-performing pairs). For monolingual data, we sampled from mC4 and MADLAD at a same 2:1 ratio (30,000 per language for better-performing languages and 15,000 per language for underperforming languages).
\subsection{SFT}












==> EMNLP-2024/sections/tmp.tex <==
% \begin{table*}[!ht]
% \centering
% \footnotesize
% \begin{tabular}{ccccccccc}
% \toprule
%          & \multicolumn{3}{c}{Reasoning} & Knowledge & \multicolumn{2}{c}{Question Answering} & Classification & Translation \\
% Systems  & mGSM    & mSVAMP    & xCSQA   & mLAMA     & XQUAD              & MLQA              & SIB-200        & Flores-101  \\
% \midrule
% TowerLLM &         &           &         &           &                    &                   &                &             \\
% Aya      &         &           &         &           &                    &                   &                &             \\
% LLaMA3   &         &           &         &           &                    &                   &                &             \\
% xLLaMA3  &         &           &         &           &                    &                   &                &             \\
% \bottomrule
% \end{tabular}
% \end{table*} 
% \subsection{Correlation between Translation Performance and downstream tasks}
% Figure ... (X-axis translation performance, Y-axis downstream task performance)
